Noise-Robust Target-Speaker Voice Activity Detection Through Self-Supervised Pretraining

Target-Speaker Voice Activity Detection (TS-VAD) is the task of detecting the presence of speech from a known target-speaker in an audio frame. Recently, deep neural network-based models have shown good performance in this task. However, training these models requires extensive labelled data, which is costly and time-consuming to obtain, particularly if generalization to unseen environments is crucial. To mitigate this, we propose a causal, Self-Supervised Learning (SSL) pretraining framework, called Denoising Autoregressive Predictive Coding (DN-APC), to enhance TS-VAD performance in noisy conditions. We also explore various speaker conditioning methods and evaluate their performance under different noisy conditions. Our experiments show that DN-APC improves performance in noisy conditions, with a general improvement of approx. 2% in both seen and unseen noise. Additionally, we find that FiLM conditioning provides the best overall performance. Representation analysis via tSNE plots reveals robust initial representations of speech and non-speech from pretraining. This underscores the effectiveness of SSL pretraining in improving the robustness and performance of TS-VAD models in noisy environments.

==> plots_and_tables/speaker_conditioning_comparison.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Noise level},
        ylabel={mAP [\si{\percent}]},
        xtick={-5, 0, 5, 10, 15, 20, 25},
        xticklabels={-5 dB, 0 dB, 5 dB, 10 dB, 15 dB, 20 dB, clean},
        ytick={50, 60, 70, 80, 90, 100},
        ymin=50, ymax=100,
        legend style={at={(0.5,-0.2)},
                      anchor=north, 
                      legend columns=2},
        grid=major
    ]

    % Extra legend entries for baseline and pretrained
    \addlegendimage{dashed, color=black}
    \addlegendentry{Base}

    \addlegendimage{solid, color=black}
    \addlegendentry{DN-APC}

    % ET category
    \addplot[dashed, mark=o, color=aaubluelight, forget plot, mark size=1pt, mark options={solid}] coordinates {
        (-5, 59.86)(0,71.42)(5,78.77)(10,82.81)(15,85.14)(20,86.60)(25,88.63)
    };
    \addplot[solid, mark=square, color=aaubluelight, mark size=1pt, mark options={solid}] coordinates {
        (-5,61.11)(0,72.53)(5,79.75)(10,83.77)(15,86.11)(20,87.57)(25,89.81)
    };
    
    % FiLM category
    \addplot[dashed, mark=o, color=aausec1, forget plot, mark size=1pt, mark options={solid}] coordinates {
        (-5, 60.80) (0, 72.27) (5, 79.49) (10, 83.47) (15, 85.72) (20, 87.09) (25, 89.11)
    };
    \addplot[solid, mark=square, color=aausec1, mark size=1pt, mark options={solid}] coordinates {
        (-5, 62.83) (0, 74.04) (5, 80.87) (10, 84.59) (15, 86.76) (20, 88.15) (25, 90.33)
    };

    % % ET2 category
    % \addplot[dashed, mark=*, color=aausec2, forget plot] coordinates {
    %     (-5, 0.15) (0, 0.25) (5, 0.35) (10, 0.45) (15, 0.55) (20, 0.65) (25, 0.75)
    % };
    % \addplot[solid, mark=*, color=aausec2] coordinates {
    %     (-5, 0.25) (0, 0.35) (5, 0.45) (10, 0.55) (15, 0.65) (20, 0.75) (25, 0.85)
    % };
    % % ET3 category
    % \addplot[dashed, mark=*, color=aausec3, forget plot] coordinates {
    %     (-5, 0.05) (0, 0.15) (5, 0.25) (10, 0.35) (15, 0.45) (20, 0.55) (25, 0.65)
    % };
    % \addplot[solid, mark=*, color=aausec3] coordinates {
    %     (-5, 0.31) (0, 0.41) (5, 0.51) (10, 0.61) (15, 0.7) (20, 0.8) (25, 0.9)
    % };

    % Legends
    \addlegendimage{solid, color=aaubluelight}
    \addlegendentry{Concat}

    % \addlegendimage{solid, color=aausec1}
    % \addlegendentry{Add}

    % \addlegendimage{solid, color=aausec2}
    % \addlegendentry{Mult.}

    \addlegendimage{solid, color=aausec3}
    \addlegendentry{FiLM}

    \end{axis}
\end{tikzpicture}
